High Dimensional Restrictive Federated Model Selection with multi-objective Bayesian Optimization over shifted distributions

A novel machine learning optimization process coined Restrictive Federated Model Selection (RFMS) is proposed under the scenario, for example, when data from healthcare units can not leave the site it is situated on and it is forbidden to carry out training algorithms on remote data sites due to either technical or privacy and trust concerns. To carry out a clinical research under this scenario, an analyst could train a machine learning model only on local data site, but it is still possible to execute a statistical query at a certain cost in the form of sending a machine learning model to some of the remote data sites and get the performance measures as feedback, maybe due to prediction being usually much cheaper. Compared to federated learning, which is optimizing the model parameters directly by carrying out training across all data sites, RFMS trains model parameters only on one local data site but optimizes hyper-parameters across other data sites jointly since hyper-parameters play an important role in machine learning performance. The aim is to get a Pareto optimal model with respective to both local and remote unseen prediction losses, which could generalize well across data sites. In this work, we specifically consider high dimensional data with shifted distributions over data sites. As an initial investigation, Bayesian Optimization especially multi-objective Bayesian Optimization is used to guide an adaptive hyper-parameter optimization process to select models under the RFMS scenario. Empirical results show that solely using the local data site to tune hyper-parameters generalizes poorly across data sites, compared to methods that utilize the local and remote performances. Furthermore, in terms of dominated hypervolumes, multi-objective Bayesian Optimization algorithms show increased performance across multiple data sites among other candidates.

==> app.tex <==
\subsection{Detail to $\fsoth$: Bayesian Optimization Combined with Thresholdout Algorihtm}\label{ap-sec:fsoth}
\urldef\urlchem\url{https://github.com/DIDSR/ThresholdoutAUC/blob/a5a3030fc53e1ab70b4e003ccc3b64cd496ec68e/functions/thresholdout_auc.R#L16}
Compared to an honest curator, $J^r_i(\phi_{i}\mid D_{cu}, D_{ob})$ = $\perf(D_{cu}\mid \theta_{i})$ in line \ref{algoline:perf} and \ref{algoline:perf2} of Algorithm \ref{algo:fmobo-ms}, Thresholdout algorithm perturbs the outcome with a noise mechanism where the unperturbed performance $\perf(D_{cu}\mid \theta_{i})$ serves as the input to the thresholdout mechanism described in \cite{Dwork2017}. The whole process is depicted in Algorithm \ref{algo:th}, where we have referenced the implementation\footnotemark\footnotetext{\urlchem} from github of \cite{Gossmann2018}. As an initial investigation, following \cite{Dwork2017,Gossmann2018}, the Laplace distribution is replaced by Gaussian, and  we used the same parameter as mentioned in section 3.1 in \cite{Gossmann2018} where the noise distribution is Gaussian, with threshold $T= 0.02$, $\sigma = 0.03$ and $\gamma = 0$. We invite the reader to refer to the reference for deeper meanings of these parameters.
\begin{algorithm}[t]
	\caption{Thresholdout-Bayesian Optimization}\label{algo:th}
	\begin{algorithmic}[1]
		\Procedure{Thresholdout-BO:}{}
		\State Input: $D_{cu}^{ig}$, $D_{ob}^{ig}$, noise rate $\sigma$, threshold $T$
		\State set $\hat{T} = T + \gamma$ for $\gamma \sim Lap(2\sigma)$, $\eta \sim Lap(4\sigma)$
		 %\Comment{Bayesian Optimization with Thresholdout}
		 \State Replace $\perf(D_{cu}\mid \theta_{i})$ in line \ref{algoline:perf} and \ref{algoline:perf2} in Algorithm \ref{algo:fmobo-ms} with the following: 
		 \If{|$\perf(D_{ob}^{ig}\mid \theta) -\perf(D_{cu}^{ig}\mid\phi)$|>T+$\eta$}
		 \State return $\perf(D_{cu}^{ig}\mid\theta) + \xi$
		 \State $\hat{T} = T + \gamma$
		 \Else{}
		 \State return $\perf(D_{ob}^{ig}\mid\theta)$
		 \EndIf
		 \State The rest of the steps remain intact as in Algorithm \ref{algo:fmobo-ms}
		 %\Else{asg}
		 %\State ag
		\EndProcedure
	\end{algorithmic}
\end{algorithm}

One possible draw back of combining Bayesian Optimization with Thresholdout is that is if $|\perf(D_{ob}^{ig}\mid \theta) -\perf(D_{cu}^{ig}\mid\phi)|$ remains to be smaller than the threshold $T+\eta$, the Bayesian Optimization does not gain further information about the response surface with regard to the curator so the search with Bayesian Optimization may become rather inefficient. Another difficulty here is that the Thresholdout family algorithm relies on the .i.i.d. distribution assumption which could be violated in most real data scenario. However, these are some initial considerations only, and we leave it for the future work to have deeper insight into this and improve upon these difficulties.



%\subsection{Model Selection on Pareto front}
%Since our multi-objective tuning returns a Pareto front, we have to figure out how to choose a single model from the Pareto front. \todo{AB: Why? For visualization?}
%\paragraph{alpha-regret selection:}
%One option is to let the user first choose a hyper-parameter $\alpha$ which decides the relative importance of his/her local dataset (the openbox) with respect to the remote dataset (in terms of both the curator and unseen lockbox). From the Pareto front, calculate the combined objective in Equation (\ref{eq:paretoselalpha}) 
%
%\begin{align}
%&J(\phi) = \alpha J_{ob} + \leftb 1-\alpha \rightb J_{cu}\nonumber\\
%\text{where,} \nonumber\\
%&J_{ob} = \perf \left(D_{ob}^{ig}\mid\theta =\hypDtom(D_{ob}^{ig}\mid \phi)\right) \nonumber   \\
%&J_{cu} = \perf \leftb D_{cu}^{ig} \mid\theta=\hypDtom(D_{ob}^{ig}\mid \phi)\rightb 
%\label{eq:paretoselalpha}
%\end{align}
%
%So we can always select the best model on the Pareto front according to Equation (\ref{eq:paretoselalpha}). We then use the same alpha here also for evaluation of performance with alpha-regret evaluation mentioned in section \ref{subsec:eval}. \todo{AB: The last sentence is unclear.}

==> commands.tex <==
%\pagestyle{plain} % removes running headers

%%head
%\usepackage[utf8]{inputenc}
\RequirePackage[utf8x]{inputenc}

\usepackage{algorithm}
%\usepackage{algorithmic}
%\usepackage[]{algorithmic} 
%\usepackage{algorithmicx}
%\usepackage[]{algorithm2e}
\usepackage{algpseudocode}
%\renewcommand{\algorithmicrequire}{}
%%%%%%%%%%%
\usepackage[export]{adjustbox}
%\usepackage[table]{xcolor}-------bug
\usepackage{amsmath}
\usepackage{mathtools}
\usepackage{relsize}
%\usepackage{breqn}
\DeclareMathOperator*{\argmax}{arg\,max}
\usepackage{float}
\usepackage{caption}
\usepackage{blindtext}
\usepackage{caption}
\usepackage{multirow}
\usepackage{microtype}
\usepackage{graphicx}
\usepackage{fixltx2e,graphicx,mathpazo}
\usepackage{subfigure}
\usepackage{booktabs} % for professional tables
\usepackage{hyperref}

% Attempt to make hyperref and algorithmic work together better:
%\newcommand{\theHalgorithm}{\arabic{algorithm}}
\usepackage{tikz}
\usetikzlibrary{calc,decorations.markings}
\usetikzlibrary{bayesnet}
\usetikzlibrary{arrows,calc,positioning,shadows,shapes}
\pgfdeclarelayer{tp}    % declare top layer
\pgfsetlayers{main, tp}  % set the order of the layers (main is the standard layer)
\usetikzlibrary{backgrounds}
\usetikzlibrary{matrix}

%\usepackage{natbib}
\usepackage[square,sort,comma,numbers]{natbib}
\usepackage{graphicx}

% comment
\usepackage{thumbpdf,lmodern}
\usepackage{placeins}
%\usepackage{todonotes}
\usepackage[colorinlistoftodos]{todonotes}
%\usepackage[left=1cm,right=1cm,top=1cm,bottom=1cm,nohead,nofoot]{geometry}
\usepackage{framed}
\newcommand{\TODO}[1]{\todo[inline]{TODO:~#1}}
\newcommand{\AB}[1]{\todo[inline]{AB:~#1}}
\newcommand{\ML}[1]{\todo[inline]{ML:~#1}}
\newcommand{\JR}[1]{\todo[inline]{JR:~#1}}
\newcommand{\XS}[1]{\todo[inline]{XS:~#1}}
\newcommand{\BB}[1]{\todo[inline]{BB:~#1}}
\newcommand{\FP}[1]{\todo[inline]{FP:~#1}}
\newcommand{\curator}{\xi}
\newcommand{\leftb}{\left(}
\newcommand{\rightb}{\right)}
\newcommand{\lefts}{\left[}
\newcommand{\rights}{\right]}
\newcommand{\rep}{\mathcal{R}}
\newcommand{\hypDtom}{\mathcal{L}}
\newcommand{\perf}{\mathcal{F}}
\newcommand{\concate}{\|}
\newcommand{\hyperv}{\mathcal{H}}
\newcommand{\eval}{\mathcal{V}}
%\newcommand{\dash}{\scalebox{0.75}[1.0]{\( - \)}}
\newcommand{\dash}{\text{-}}
\newcommand{\fsoth}{\textbf{fso\_th}}
\newcommand{\lso}{\textbf{lso}}
\newcommand{\fso}{\textbf{fso}}
\newcommand{\fmo}{\textbf{fmo}}
\newcommand{\randmo}{\textbf{rand\_mo}}
\newcommand{\mfig}[5]{
	\begin{figure}[#5]
		\centering
		\includegraphics[scale=#4]{#1}
		\caption{#2}
		\label{fig:#3}
\end{figure}}


\newcommand{\mgraph}[4]{
	\centering
	\includegraphics[width=1\textwidth, scale=#4]{#1}
	\caption{#2}
	\label{#3}}

